Restart-Based Fault-Tolerance: System Design and Schedulability Analysis

Embedded systems in safety-critical environments are continuously required to deliver more performance and functionality, while expected to provide verified safety guarantees. Nonetheless, platform-wide software verification (required for safety) is often expensive. Therefore, design methods that enable utilization of components such as real-time operating systems (RTOS), without requiring their correctness to guarantee safety, is necessary. In this paper, we propose a design approach to deploy safe-by-design embedded systems. To attain this goal, we rely on a small core of verified software to handle faults in applications and RTOS and recover from them while ensuring that timing constraints of safety-critical tasks are always satisfied. Faults are detected by monitoring the application timing and fault-recovery is achieved via full platform restart and software reload, enabled by the short restart time of embedded systems. Schedulability analysis is used to ensure that the timing constraints of critical plant control tasks are always satisfied in spite of faults and consequent restarts. We derive schedulability results for four restart-tolerant task models. We use a simulator to evaluate and compare the performance of the considered scheduling models.

==> Sections/implementation.tex <==

\section{Proof-Of-Concept Implementation}


\subsection{3DOF helicopter and Controllers}

The 3DOF helicopter~(displayed in figure~\ref{fig:3dof}) is a
simplified helicopter model, ideally suited to test intermediate to
advanced control concepts and theories relevant to real world
applications of flight dynamics and control in the tandem rotor
helicopters, or any device with similar
dynamics~\cite{3dofhelicopter}. It is equipped with two motors that
can generate force in the upward and downward direction,
proportionally to the given actuation voltage. It also has three
sensors to measure elevation, pitch and travel angle as shown in
Figure~\ref{fig:3dof}.

\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=0.35\textwidth]{dof}
		\caption{3 Degree of freedom~(3DOF) helicopter.}
		\label{fig:3dof}
	\end{center}
\end{figure}




\begin{table*}[]
	\centering
	\small
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		\multicolumn{6}{|c|}{3DOF Helicopter Fault Injection}                         \\ \hline
		\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} }                                        & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} }                                                                                    & \multicolumn{3}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} Safety}}                                                                                                                                                                                                                      & \cellcolor[HTML]{C0C0C0}                                     \\ \cline{3-5}
		\multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} \textbf{Failure Type}}} & \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}c@{}}Fault\\ Category\end{tabular}}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}Application-Level\\ Simplex\\(1 processing unit)\end{tabular}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}System-Level\\ Simplex\\ (2 processing units)\end{tabular}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}Our Approach\\ (1 processing unit)\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{Restarted}} \\ \hline
		\cellcolor[HTML]{EFEFEF}No Output                                                      & App.                                                                                                                        & \cmark                                                                                                                 & \cmark                                                                                                           & \cmark                                                          & No                                                           \\ \hline
		\cellcolor[HTML]{EFEFEF}Maximum Voltage                                     & App.                                                                                                                        & \cmark                                                                                                                 & \cmark                                                                                                           & \cmark                                                          & No                                                           \\ \hline
		\cellcolor[HTML]{EFEFEF}Time Degraded Control                                          & App.                                                                                                                        & \cmark                                                                                                                 & \cmark                                                                                                           & \cmark                                                          & No                                                           \\ \hline
		% \cellcolor[HTML]{EFEFEF}Resource Exhaustion                                            & OS/App.                                                                                                                     & \xmark                                                                                                                 & \cmark                                                                                                           & \cmark                                                          & Yes                                                          \\ \hline
		\cellcolor[HTML]{EFEFEF}Resource Blocking - CPU                                                 & RTOS/App.                                                                                                                     & \xmark                                                                                                                & \cmark                                                                                                           & \cmark                                                          & Yes                                                          \\ \hline
		\cellcolor[HTML]{EFEFEF}Resource Blocking - Port                                                  & RTOS/App.                                                                                                                     & \xmark                                                                                                                & \cmark                                                                                                           & \cmark                                                          & Yes                                                          \\ \hline
		\cellcolor[HTML]{EFEFEF}FreeRTOS Freeze                                                      & RTOS                                                                                                                                 & \xmark                                                                                                                & \cmark                                                                                                           & \cmark                                                          & Yes                                                          \\ \hline
		\cellcolor[HTML]{EFEFEF}CPU Reboot                                                & RTOS                                                                                                                                 & \xmark                                                                                                                & \cmark                                                                                                           & \cmark                                                          & Yes                                                          \\ \hline
		
	\end{tabular}
	\caption{Our approach tolerates the system-level faults using only one processing unit. Whereas, System-Level Simplex~\cite{bak2009system} needs an extra processing unit to tolerate these faults.}
	\label{table:tests}
\end{table*}


Safety for the 3DOF helicopter is achieved if the propellers do not
hit the surface underneath, as shown in Figure~\ref{fig:3dof}. The
subset of the state space in which there is no contact between the
helicopter and the surface underneath is given by $-\epsilon -\rho/3
\leq 0.3$ and $-\epsilon +\rho/3 \leq 0.3$ where $\epsilon$ and $\rho$
are the elevation and pitch angles of the helicopter. The helicopter
is considered safe if it never exits this region. To design the
decision logic and the safety controller, we use the Simplex-based
approach proposed in~\cite{rt-reach} and the linear model of 3DOF
helicopter obtained from the manufacturer
manual~\cite{3dofhelicopter}. We also design a complex controller that
makes the helicopter follow a set of circular set points The logic of
the complex controller is not safe, i.e. as it control the plant to
follow the set points, the helicopter may hit the surface.


%Equation~(\ref{eq:voltageLimit}) describes the limits on the motor voltages of the helicopter in the form of $H_u \cdot u \leq h_u$.
%
%\begin{equation}
%\label{eq:voltageLimit}
%\left[
%\begin{array}{cc}
%1& 0\\
%-1 & 0\\
%0& 1\\
%0& -1\\
%\end{array}
%\right]
%\left[
%\begin{array}{c}
%v_l\\
%v_r\\
%\end{array}
%\right] \leq
%\left[
%\begin{array}{c}
%1.1\\
%1.1\\
%1.1\\
%1.1\\
%\end{array}
%\right]
%\end{equation}
%
%Here, $v_l$ and $v_r$ are the voltage for controlling left and right motors.

\subsection{Controller Implementation}

For the prototype of the proposed design, a Freescale i.MX7D
application processor is considered. This SoC provides two general
purpose ARM Cortex-A7 cores capable of running at the maximum
frequency of 1~GHz and one real-time ARM Cortex-M4 core that runs at
the maximum frequency of 200~MHz. The real-time core runs from tightly
coupled memory to ensure predictable behavior required for real-time
applications/tasks. The real-time core on the considered platform runs
FreeRTOS~\footnote{http://www.freertos.org}, a popular open-source
real-time operating system.

Due to the real-time constraints of the control tasks, we choose the
real-time ARM Cortex-M4 core to run the controller. Faults occurring
on ARM Cortex-M4 core trigger a full restart of the ARM Cortex-M4 core
followed by a full reload of the image containing the OS (FreeRTOS)
and the control software. On the i.MX7D platform, only the Cortex-A7
cores have direct access to the flash memory, and only these two cores
are responsible for loading the binary images of the real-time core
from flash. The first time after a platform bootstrap, the image of
the FreeRTOS and the control software is loaded into the RAM of the
Cortex-A7 cores. Every time the real-time core restarts, the FreeRTOS
and control applications are loaded into real-time core's tightly
coupled memory by any of the Cortex-A7 cores. This procedure also
reduces the restart-time of the real-time core as it does not have to
read the image from flash memory~(which is usually slower than
RAM). With the above implementation, the restart time of the real-time
core is less than 1ms\footnote{SC task activates one of the GPIO pins
  immediately after it executes. The restart time is measured
  externally using the signal on this pin. After multiple experiments,
  a conservative upper bound was picked for the restart time.}.

The control tasks~(SC, CC, and DM tasks) on the ARM Cortex-M4 core run
with a frequency of 50~Hz~(\ie period of 20~ms). Our controller
interfaces with the 3DOF helicopter through a PCIe-based \textit{Q8
  High-Performance H.I.L. Control and data acquisition
  unit}~\cite{q8daq} and an intermediate Linux-based PC. The PC
communicates with the i.MX7D through a serial port and uses a custom
Linux driver for sending the voltages to the 3DOF helicopter motors
and reading the sensor values. Inside FreeRTOS, a task periodically
checks if the SC and DM tasks have completed before their response
time, and it updates the WD timer accordingly. Otherwise, the WD
expires, triggering a restart of real-time core. After the completion
instant of every task, the scheduler state is stored in a fixed
address of the Cortex-A7 RAM. Notice that the Cortex-A7 RAM is not
impacted by restarting the Cortex-M4 core. Therefore, after the
restart of Cortext-M4 core, the scheduler state can retrieved from the
system RAM of Cortex A7 cores.

% the stored state and continue operation. 



% At the end of every control cycle, a flushing task on the real-time
% core communicates with the PC to receive the sensor
% readings~(elevation, pitch, and travel angles) and send the motors'
% voltages. It also updates the hardware WD of the platform after
% sending the motor voltages.


% Note that, this mechanism is specific to this particular platform
% and does not impact the generality of our proposed technique.

% The real-time core on the considered SoC is not capable of booting
% at its own because it does not have a flash memory. It is the
% responsibility of the general purpose core to load the code of the
% real-time core in its memory and release it from the reset. This
% mechanism is specific to this particular platform and does not
% impact the generality of our proposed solution.

% The original boot procedure of the board is as follows: At boot time
% the general purpose processor copies the bootloader (u-boot) from
% the SD-card into the RAM; this bootloader later copies the kernel
% from the SD-card into the RAM and passes control to the kernel; and
% the kernel later mounts the filesystem present in one of the
% partition of the SD-card which then provides the control of the
% general purpose processor using a Linux terminal over UART.

% The manufacturer's boot procedure of the board is designed to boot
% the general purpose cores and the real-time core at the same
% time. It includes extra initialization procedures that are necessary
% only for running the general purpose core's kernel and mounting its
% file system. It loads the real-time core code only after those
% procedures are completed.


% To reduce the boot time of the real-time core, we made two
% modifications to the bootloader~(u-boot) source code which can be
% found in~\cite{githubrepo-address}. \hl{TODO: upload the final code
% on github and cite} \ci~We included the binary of the real-time core
% executables~(FreeRTOS, MC, BC, DM, and flushing task) as a static
% array in the u-boot source code and made it part of the u-boot
% binary after compilation. \cii~In our modified boot process, at the
% boot time, the general purpose processor copies u-boot binary~(that
% includes the FreeRTOS and application binaries) from the SD-card
% into the RAM. After successful initialization of only the necessary
% peripherals and configuring the clock by the u-boot procedures,
% u-boot loads the binaries of the real-time core in its tightly
% coupled memory and releases it from reset. These modifications
% reduce the real-time core's boot time from seconds to less than
% 250ms\footnote{BC task activates one of the GPIO pins immediately
% after it executes. The restart time is measured externally using the
% signal on this pin. After multiple experiments, a conservative upper
% bound was picked for the restart time.}.



% U-boot then loads the image of the real-time core from RAM into the
% tightly coupled memory of the real-time core.


% We have used a commercial off-the-shelf i.MX7D application platform
% to implement our controller.  This platform provides two general
% purpose ARM Cortex-A7 cores and one Cortex-M4 core which runs from a
% tightly coupled memory to ensure the predictable behavior required
% for real-time functionality. The Cortex M4 runs
% FreeRTOS~\cite{freertos} that provides real-time functionality.  We
% have implemented our complex controller on the real-time Cortex-M4
% core of i.MX7D\footnote{ In i.MX7D chips, only Cortex-A7 cores have
% access to the permanent storage. Therefore, we need the Cortex-A7
% core to load the image to the memory of the real-time Cortex-M4
% core. This however, is a limitation of this particular platform and
% does not impact the generality of the solution.}.

% The current u-boot implementation provided for the Cortex A7 core
% has a "bootaux" command that helps with booting the Cortex M4
% core. However, using that command at least takes two seconds to boot
% the Cortex-M4 core because it first loads the


% In order to reduce the boot time of the real-time core, we made
% several modifications to the the u-boot source code. Originally,
% u-boot initializes all the peripherals first, and then reads the
% binary file of the OS and controllers from the SD-card and loads it
% into the memory of the real-time core. The first modification that
% we made is to integrate the binray image of the OS and controllers
% as an static array with u-boot source code and make it part of the
% u-boot binary after compilation. This loads the the OS and
% controller binary along with the u-boot into the RAM at boot
% time. Second, after the u-boot has finished configuring the clocks
% to different peripherals, the first thing that we do is to load the
% OS and controller image to Cortex-M4 memory and release it from
% reset. Doing these optimization helped us to boot the FreeRTOS on
% the Cortex-M4 core in less than 250 ms. %

% To integrate the reset based mechanism onto the real-time core
% running mission controller, we relied on watchdog timer present on
% the chip. At any if the watchdog detects that the core is stuck it
% performs a system-wide reset and the whole system comes back in 250
% ms.

% Furthermore, in order to protect the image on the SD-card we set it
% as an read-only partition. This will protect the image from being
% modified\footnote{Complex OS faults could possibly ignore the
% read-only partition limit and modify the image. We are working on a
% HW enforced read-only storage for the future implementations.}.

\subsection{Fault Injection}

Table~\ref{table:tests} presents a list of faults that we tested on
our implemented controller. For the investigated system-level faults,
we observed that the WD timer restarted the system, the safety
controller task did not miss the deadline after restart, and the
physical system remained in safe state. For application faults, we
observed that when the helicopter's state approached potentially
unsafe states, as a result of faults or unsafe logic in complex
controller, the DM detected the safety hazard and switched the control
to safety controller. This prevented the helicopter from crashing.

To provide a comparison point, we provide the performance of
Application-Level Simplex and System-Level Simplex. As shown in
Table~\ref{table:tests}, System-Level Simplex is able to tolerate all
the system-level and application-level faults because, due to hardware
isolation, backup controller is not impacted by the system-level
faults on the complex subsystem. Whereas our proposed approach does
not require any additional hardware.


% For the application-level faults, we observed that the SC task was
% able to actuate the 3DOF helicopter as long as it did not jeopardize
% safety. When the helicopter’s state approached the states where the
% safety conditions were not satisfied, BC took over and prevented the
% helicopter from hitting the surface underneath.

In the rest of this section, we elaborate some of these faults. 

% Please add the following required packages to your document
% preamble: \usepackage[table,xcdraw]{xcolor} If you use beamer only
% pass "xcolor=table" option,
% i.e. \documentclass[xcolor=table]{beamer} Please add the following
% required packages to your document preamble: \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor} If you use beamer only pass
% "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\subsubsection{Maximum Voltage in Wrong Way}
The helicopter should not hit the surface even if the CC outputs a
voltage that normally would result in a crash. We consider an extreme
case of this scenario where the CC generates a voltage that pushes the
helicopter towards the surface. The unsafe CC commands were detected
by DM, and the control was switched to the SC until the helicopter was
in the safety and then control was handed back to CC.



% In this test, some processes other than BC and DM have memory
% leak. Over the time they prevent the safety-critical tasks such as
% DM and BC from executing on time.


% In order to implement and test this scenario. After fives seconds of
% run from the reset, we introduce another task that runs at the same
% priority as the BC and DM but it steals some of the CPU cycles of
% both the tasks which eventually triggers the watchdog to issue
% system wide reset since both DM and BC task miss their deadline.

% \hl{@Rohan: Due to OS faults one task is scheduled multiple times
% and therefore there are no CPU cycles and BC or DM cannot run.}



\subsubsection{Blocking Shared Resource}
A faulty process may behave differently in runtime from its
expected/reported behavior. For instance, it may lock a particular
resource which is also needed by other critical tasks for more than
the intended duration. Or, it may execute for more time than its
reported WCET that is used for the schedulability test of the
system. These faults may also originate from RTOS or driver
misbehavior due to race condition or other reasons. If the fault
delays/stops the execution of the DM or SC, WD will trigger a
system-wide restart. This recovers the system from the fault and keeps
the physical system safe. We perform two experiments to test the
fault-tolerance against this category of faults.

In the first experiment, we added an additional task to the system
that uses the serial port in parallel to the SC task to communicate
with the PC. We injected a fault into this task such that in random
execution cycles, it holds the lock on the serial port for more than
the intended period. This prevents the SC task from sending the
control command~(for which it requires the serial port). As a result,
WD expires and restarts the system. We observed that the system
recovered from the fault and remained safe during the restart.

% All the tasks scheduled on the system compete for the same
% resources~(\eg CPU cycles, memory) and they can prevent the
% safety-critical tasks from timely execution if misuse those
% resources.

In the second test, we introduced a task that runs at the same
priority as the SC and DM. We injected a fault, into the task such
that in some cycles, its execution time exceeds its reported
WCET. FreeRTOS runs the tasks with equal priority using round-robin
scheduling with a context switch at every 1ms. Therefore, the faulty
task delays the response time of the DM and SC. If the interference is
too long, the output of SC may not be ready by the time, the flushing
task needs to update the actuators. When this happened, WD restarted
the system.

